The Survival and Entrainment of Molecules and Dust in Galactic Winds

Recent years have seen excellent progress in modeling the entrainment of T $\sim$ $10^4$K atomic gas in galactic winds. However, the entrainment of cool, dusty T $\sim$ 10-100K molecular gas, which is also observed outflowing at high velocity, is much less understood. Such gas, which can be $10^5$ times denser than the hot wind, appears extremely difficult to entrain. We run 3D wind-tunnel simulations with photoionization self-shielding and evolve thermal dust sputtering and growth. Unlike almost all such simulations to date, we do not enforce any artificial temperature floor. We find efficient molecular gas formation and entrainment, as well as dust survival and growth through accretion. Key to this success is the formation of large amounts of 10^4K atomic gas via mixing, which acts as a protective "bubble wrap" and reduces the cloud overdensity to $\sim$ 100. This can be understood from the ratio of the mixing to cooling time. Before entrainment, when shear is large, t_mix/t_cool $\leq$ 1, and gas cannot cool below the "cooling bottleneck" at 5000K. Thus, the cloud survival criterion is identical to the well-studied purely atomic case. After entrainment, when shear falls, t_mix/t_cool > 1, and the cloud becomes multi-phase, with comparable molecular and atomic masses. The broad temperature PDF, with abundant gas in the formally unstable 50 K < T < 5000 K range, agrees with previous ISM simulations with driven turbulence and radiative cooling. Our findings have implications for dusty molecular gas in stellar and AGN outflows, cluster filaments, "jellyfish" galaxies and AGB winds.

==> scratch.tex <==
\subsection{Cloud Survival Criterion} \label{sec:cloud survival criterion}

To study the {\it long-term} survival of molecular gas and dust in clouds, the bottom line is that the original cloud needs to survive the wind acceleration and get entrained. Otherwise any molecular gas that might have formed will eventually get destroyed. We briefly review the survival criterion of optically thin atomic clouds, which turns out to work remarkably well for our molecular clouds. We will discuss why this is the case in \autoref{sec:intermediate cloud} and present some new insights about the cloud survival criterion in \autoref{sec:Survival Criterion for Clouds with Molecules}.

The survival of optically thin, atomic-temperature ($10^4 {\rm K}$) clouds in hot winds boils down to a competition between the destruction of the cloud due to instabilities introduced by the wind and the replenishment of cloud material by radiative cooling \citep{gronke18}. Each of the two competing processes can be quantified by a corresponding timescale. \citep{gronke18} were one of the first to tackle this cloud survival problem. They quantified the timescale for cloud destruction by the cloud-crushing time $t_{\rm cc}$, given by 

\begin{align}
    t_{\rm cc} \sim \chi^{1/2} \frac{r_{\rm initial}}{v_{\rm wind}} \label{eq:t_cc}
\end{align}

where $\chi = \left. \rho_{\rm cloud} \right/ \rho_{\rm wind}$ is the density contrast between the cloud and the wind, $r_{\rm initial}$ is the initial radius of the cloud, and $v_{\rm wind}$ is the initial wind velocity relative to the cloud. On the other hand, the replenishment of cold cloud material can be described by the radiative cooling time of the mixed gas at the cloud-wind interface, which is given by 

\begin{align}
    t_{\rm cool,mix} = t_{\rm cool,isobaric} \left(T_{\rm mix}\right) = t_{\rm cool,isobaric} \left(\sqrt{T_{\rm cloud} T_{\rm wind}}\right)\label{eq:t_cool,mix},
\end{align}

where we evaluate the isobaric cooling time at the mixed gas temperature $T_{\rm mix}$.

\cite{gronke18} argued that if $\left. t_{\rm cool,mix} \right/ t_{\rm cc} \ll 1$, radiative cooling of the mixed gas is sufficiently efficient such that new, co-moving gas at atomic temperatures ($10^4 {\rm K}$) can be generated at the tail of the cloud. This leads to an entrained cloud that grows by an order of magnitude in mass. \cite{gronke18} recast the cloud survival criterion $\left. t_{\rm cool,mix} \right/ t_{\rm cc} \ll 1$ into a critical initial radius for cloud survival, given by

\begin{align}
   r_{\rm crit} &= \frac{v_{\rm wind} t_{\rm cool,mix}}{\chi^{1/2}} \alpha_{\rm crit}^{-1} \nonumber \\
   &= 2 {\rm pc} \frac{T_{\rm cl,4}^{\left. 5\right/2} \mathcal{M}_{\rm wind}}{P_{\rm 3} \Lambda_{\rm mix,-21.4}} \frac{\chi}{100} \alpha_{\rm crit}^{-1},  \label{eq:cloud survival radius}
\end{align}

where $T_{\rm cl,4} \equiv \left. T_{\rm cl} \right/ 10^4 \: {\rm K}$, $P_{\rm 3} \equiv \left. nT \right/ \left(10^3 {\rm cm}^{-3} \: {\rm K}\right)$, $\Lambda_{\rm mix,-21.4} \equiv \left. \Lambda_{\left(T_{\rm mix}\right)} \right/ \left(10^{-21.4} \: {\rm erg} \: {\rm cm}^3 \: {\rm s}^{-1}\right)$, $\mathcal{M}_{\rm wind}$ is the Mach number of the hot wind, and $\alpha_{\rm crit}$ is the value of $\left.t_{\rm cool,mix} \right/t_{\rm cc}$ at the critical survival radius $r_{\rm crit}$. We note here that the value of $\alpha_{\rm crit}$ needs to be empirically calibrated and can be different from different choices of $T_{\rm cl}$. 

More recently, \cite{Abruzzo:2023} modified this timescale argument for cloud survival to come up with a unified survival criterion. Their crucial insight is that cloud can only grow if an incoming parcel of hot gas can mix and cool down to the cloud temperature before it is advected past the cloud. Thus, the timescale that should be compared to the radiative cooling time is 

\begin{align}
    t_{\rm shear} = \left. R_{\rm cl} \right./ v_{\rm wind}. \label{eq:t_shear}
\end{align}

At the same time, they also used a slightly different cooling time given by

\begin{align}
    t_{\rm cool,minmix} = t_{\rm cool,isobaric} \left(T_{\rm minmix}\right) = t_{\rm cool,isobaric} \left(\sqrt{T_{\rm min,cool} T_{\rm wind}}\right), \label{eq:t_cool,minmix}
\end{align}

which is also used by \cite{farber22}. 

Putting things together, \cite{Abruzzo:2023} expresses the critical cloud radius for survival as

\begin{align}
    r_{\rm crit} &= \left. c_{\rm s,cold} \mathcal{M}_{\rm wind} \sqrt{\chi} t_{\rm cool,minmix} \right./ \alpha \nonumber \\
    &= 20{\rm pc} \frac{T_{\rm cl,4}^{\left. 3\right/2} \mathcal{M}_{\rm wind}}{P_{\rm 3}\Lambda_{\rm mix,-21.4}} \left(\frac{\chi}{100}\right)^{\left. 3\right/2} \left( \frac{\alpha}{7}\right)^{-1}, \label{eq:r_crit abruzzo}
\end{align}

(this is just a restatement of equation 11 in \cite{Abruzzo:2023}) or

\begin{align}
    N_{\rm crit} = 6.17 \times 10^{18} {\rm cm}^{-2} n_{-1} \frac{T_{\rm cl,4}^{\left. 3\right/2} \mathcal{M}_{\rm wind}}{P_{\rm 3} \Lambda_{\rm mix,-21.4}} \left(\frac{\chi}{100}\right)^{\left. 3\right/2} \left( \frac{\alpha}{7}\right)^{-1}, \label{eq:N_crit abruzzo}
\end{align}

where $\alpha$ is a constant that is calibrated to be $\sim$7 based on their results.

We find the survival criterion of \cite{Abruzzo:2023} to work surprisingly well in our setup. This seems counter-intuitive given that we allow cooling down to molecular temperatures. However, it is crucial to keep in mind that the cloud survival criterion is most sensitive to the \emph{average} density contrast $\chi$ of the cloud \emph{during} entrainment. As we will show in \autoref{sec:intermediate cloud}, our clouds are mostly atomic during entrainment, which means the cloud overdensity is $\sim$100. This resembles the setups of \cite{gronke18} and \cite{Abruzzo:2023} and facilitates cloud survival. The entrained cloud does cool down to molecular temperatures in its interior and has a significantly higher overdensity, but the behavior \emph{after} entrainment has no bearing to cloud survival. We will discuss the key stages of cloud evolution in more details in \autoref{sec:intermediate cloud}.

With this understanding, we can plug our parameter choices into \autoref{eq:r_crit abruzzo} (remember $\mathcal{M}_{\rm wind} = 1.5$) to find that $r_{\rm crit} \sim 30$pc. 

A crucial dimensionless ratio that determines the percentage of the optically thin "skin" in the entire cloud is $N_{\rm crit}/N_{\rm skin}$. Combining \autoref{eq:N_crit abruzzo} and \autoref{eq:self-shielding column} and plugging in our parameter choices, we find that 

\begin{align}
    N_{\rm crit}/N_{\rm skin} \sim 1. \label{eq:r_crit over d_skin}
\end{align}

Note that $N_{\rm crit}$ is the critical \emph{initial} column density for cloud survival. As the cloud gets accelerated by the wind, it becomes elongated, which means it takes some time for the transverse column density of the entrained cloud to reach the initial column density. Thus, although a $N_{\rm initial} = N_{\rm crit}$ cloud is able to survive, get entrained, and eventually become optically thick to produce molecular gas, we expect this process to take a long time. For this reason, we will focus on cloud with larger initial column densities (and radii) in the remainder of \autoref{sec:results}.

In the following sections, we analyze the survival and evolution molecules and dust in our clouds. We focus on a $r_{\rm initial} = 10 r_{\rm crit}$ cloud in \autoref{sec:intermediate cloud} but also discus smaller and larger clouds with $r_{\rm initial} = 3$ and $10 r_{\rm crit}$ respectively. 

%%%In this section, we explore how this insight allows us to revise cloud survival criterion originally developed for atomic clouds.

%The survival of optically thin atomic clouds in hot winds boils down to a competition between some cloud destruction timescale ({\cite{gronke18}} used the cloud-crushing time, while \cite{Abruzzo:2023} used the time needed for a parcel of hot gas to be advected through one cloud radius) and the cooling time of the mixed gas produced at the skin of the cloud. What we mean by "mixed gas", or at what temperature should the cooling time be evaluated at, has been a hot topic of debate in the literature. Instead of diving into this debate, we briefly discuss how the current survival criterion applies to our molecular clouds.

%%%When talking about the cooling time of the "mixed gas", it is easy to be deceived by the huge dynamical range in our simulations. In a simulation containing gas ranging from 10K to $10^6$K, it seems like the mixed gas should be roughly at the geometric mean of the extreme temperatures. However, as we have analyzed extensively in preceding sections, the cloud is predominantly atomic during entrainment, and due to photoionization, it is always atomic gas that directly interacts with the hot wind. For these reasons, we propose that the "mixed gas" whose cooling time determines cloud survival should still be between $10^4$K to $10^6$K, identical to the treatment in atomic cloud-crushing simulations. By the same logic, the density contrast $\chi$, which goes into calculating the cloud-crushing time, should be 100, not $10^5$. We have seen ample evidence of the cloud regulating its average overdensity at 100 in our simulations.

% Do the existing survival criterion for atomic clouds correctly predict this outcome? 

%First consider the survival criterion in \cite{gronke18}. Since the top left panel of \autoref{fig:medium_cloud_modified_power_law_cooling} shows that the average density contrast of the cloud is maintained about about 100 before the cloud starts to get sheared away in the wind, we take $\chi = 100$ in our calculation of the cloud-crushing time $t_{\rm cc}$, which yields

%\begin{align}
%    t_{\rm cc} \sim \chi^{1/2} \frac{r_{\rm initial}}{v_{\rm wind}} = 100^{1/2} \frac{300 {\rm pc}}{1.5 c_{\rm s,hot}} = 13.1 {\rm Myrs}.
\end{align}

%As for the cooling time of the mixed gas, since the initial cloud contains a molecular core at the temperature floor (see first temperature slice in \autoref{fig:medium_cloud_modified_power_law_cooling}), naively one would think that the cooling time should be evaluated at the geometric mean of the wind temperature and the temperature floor, which yields

%\begin{align}
%    t_{\rm cool,mix} = t_{\rm cool} (T_{\rm mix}) = t_{\rm cool} (\sqrt{T_{\rm cloud}T_{\rm wind}}) \nonumber \\ 
%    = t_{\rm cool} (\sqrt{10{\rm K} \times 10^6{\rm K}}) = 0.26 {\rm Myrs}.
%\end{align}

%Putting these together, we have

%\begin{align}
%    \frac{t_{\rm cool,mix}}{t_{\rm cc}} = \frac{0.26 {\rm Myrs}}{19.6 {\rm Myrs}} \ll 1,
%\end{align}

%which predicts cloud survival, contradictory to our simulation results. Note that if we instead take $T_{\rm cloud} = 10^4$K, the temperature of the atomic skin, then $T_{\rm mix} = 10^5$K and $t_{\rm cool,mix}$ is boosted to 4.63Myrs. Although this still predicts cloud survival (which is incorrect), it is probably a more physical choice given that it is always atomic gas that directly interacts with the wind. \textcolor{red}{ZIRUI: I did not write about that $\alpha$ factor which can be different depending on te temperature floor. Should we mention that?}

%On the other hand, following \cite{Abruzzo:2023}, we have

%\begin{align}
%    t_{\rm shear} = \frac{R_{\rm cl}}{v_{\rm wind}} = \frac{300 {\rm pc}}{1.5 c_{\rm s,hot}} = 1.96 {\rm Myrs},
%\end{align}

and

\begin{align}
    t_{\rm cool,minmix} = t_{\rm cool} (\sqrt{T_{\rm min,cool}T_{\rm wind}}) \nonumber \\ 
    = t_{\rm cool} (\sqrt{31.6{\rm K} \times 10^6{\rm K}}) = 0.43 {\rm Myrs}.
\end{align}

This means $\left. t_{\rm shear} \right/ t_{\rm cool,minmix} < 1$ and would imply cloud survival, which is incorrect. However, if we ignore the temperature at which the cooling time profile has a minimum and instead simply evaluate $t_{\rm cool}$ at the mixed temperature between atomic gas and the wind ($10^5$K), this yields $t_{\rm cool,mix}$= 4.63Myrs and $\left. t_{\rm shear} \right/ t_{\rm cool,minmix} > 1$, which correctly predicts destruction. We note here that \citep{Abruzzo:2023} also included a dimensionless parameter $\alpha$ in their survival criterion and calibrated it to be 7 in the atomic temperature ranges. Whether or not this value of $\alpha$ holds once we include the full dynamic range of temperatures is unclear.

